Dynamic Low-light Imaging with Quanta Image Sensors

Imaging in low light is difficult because the number of photons arriving at the sensor is low. Imaging dynamic scenes in low-light environments is even more difficult because as the scene moves, pixels in adjacent frames need to be aligned before they can be denoised. Conventional CMOS image sensors (CIS) are at a particular disadvantage in dynamic low-light settings because the exposure cannot be too short lest the read noise overwhelms the signal. We propose a solution using Quanta Image Sensors (QIS) and present a new image reconstruction algorithm. QIS are single-photon image sensors with photon counting capabilities. Studies over the past decade have confirmed the effectiveness of QIS for low-light imaging but reconstruction algorithms for dynamic scenes in low light remain an open problem. We fill the gap by proposing a student-teacher training protocol that transfers knowledge from a motion teacher and a denoising teacher to a student network. We show that dynamic scenes can be reconstructed from a burst of frames at a photon level of 1 photon per pixel per frame. Experimental results confirm the advantages of the proposed method compared to existing methods.

==> TeX/customFigureMacros.tex <==
% ===========================================================
% Definitions, commands and environnments for drawing figures
%
% Vivek Goyal
% based on work by
% Ivana Jovanovic, Patrick Vandewalle, Olivier Roy - 2005
% ===========================================================

% --------
% PACKAGES
% --------
%\RequirePackage{amsmath}
%\RequirePackage{amssymb}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{ifthen}
%\RequirePackage{pstricks}
%\RequirePackage{pst-plot}
%\RequirePackage{algo}
%\RequirePackage{epsfig}
%\RequirePackage{latexsym}
%\RequirePackage{subfigure}

% --------------------
% PSTRICKS DEFINITIONS
% --------------------
% Upsampling operation (reference point at the center of the circle)
% Parameter #1: upsampling factor
\def\upsampling#1{

    \pscircle(0,0){0.5}
    \psline{->}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Downsampling operation (reference point at the center of the circle)
% Parameter #1: downsampling factor
\def\downsampling#1{

    \pscircle(0,0){0.5}
    \psline{<-}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Sampling operation (reference point at the center of the box)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\sampler#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.6,-0.2)(-0.2,-0.2)
    \psline{-}(0.2,-0.2)(0.6,-0.2)
    \psline{-}(-0.2,-0.2)(0.1,0.1)
    \rput(-0.3,0.3){#1}

}

% Discrete-to-continuous operation (reference point at the center of the box)
% (Generation of weighted Dirac train)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\diracTrain#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.8,0)(0.8,0)
    \psline{->}(-0.6,0)(-0.6,-0.45)
    \psline{->}(-0.3,0)(-0.3,-0.3)
    \psline{->}( 0.0,0)( 0.0, 0.4)
    \psline{->}( 0.3,0)( 0.3, 0.4)
    \psline{->}( 0.6,0)( 0.6,-0.35)
    \rput(0.3,-0.2){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\filter#1{

    \psframe(-1,-0.5)(1,0.5)
    \rput(0,0){#1}

}

\def\shortfilter#1{

    \psframe(-0.75,-0.5)(0.75,0.5)
    \rput(0,0){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\widefilter#1{

    \psframe(-2,-0.5)(2,0.5)
    \rput(0,0){#1}

}

% Sum (reference point at the center of the circle)
\def\sumsymbol{

    \pscircle(0,0){0.25}
    \rput(0,0){$+$}

}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\analysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\downsampling{#2}}
    \psline{-}(4,0)(4.5,0)
}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\wideanalysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(2.5,0){\widefilter{#1}}
    \psline{-}(4.5,0)(5,0)
    \rput(5.5,0){\downsampling{#2}}
    \psline{-}(6,0)(6.5,0)
}

% Synthesis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: synthesis filter label
% Parameter #2: upsampling factor
\def\synthesis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(3,0){\filter{#1}}
    \psline{-}(4,0)(4.5,0)
}

% Filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: synthesis filter label
% Parameter #3: down/upsampling factor
\def\filterbankchannel#1#2#3{

    \rput(0,0){\analysis{#1}{#3}}
    \rput(4.5,0){\synthesis{#2}{#3}}

}

% Two channel filter bank (reference point at the begining of the filter bank)
% Parameter #1: lowpass analysis filter label
% Parameter #2: lowpass synthesis filter label
% Parameter #3: highpass analysis filter label
% Parameter #4: highpass synthesis filter label

\def\twochannelfilterbank#1#2#3#4{

    % Input
    \psline{*-}(0,0)(0.5,0)
    \psline{-}(0.5,-0.75)(0.5,0.75)

    % Highpass branch
    \rput(0.5,0.75){\filterbankbranch{#3}{#4}{2}}

    % Lowpass branch
    \rput(0.5,-0.75){\filterbankbranch{#1}{#2}{2}}

    % Output
    \psline{->}(9.5,0.75)(9.5,0.25)
    \rput(9.5,0){\sumsymbol}
    \psline{->}(9.5,-0.75)(9.5,-0.25)
    \psline{-*}(9.75,0)(10.25,0)

}




% Parameter #1: filter label
% Parameter #2: sampling factor
% Parameter #3: delay
\def\mybranch#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(2.75,0){\shortfilter{#3}}
    \psline{-}(3.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchA#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}


\def\mybranchB#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(4.5,0)
    \rput(5.25,0){\shortfilter{#3}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchC#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}
